Using Process Models to understand Security Standards

Many industrial software development processes today have to comply with security standards such as the IEC~62443-4-1. These standards, written in natural language, are ambiguous and complex to understand. This is especially true for non-security experts. Security practitioners thus invest much effort into comprehending standards and, later, into introducing them to development teams. However, our experience in the industry shows that development practitioners might very well also read such standards, but nevertheless end up inviting experts for interpretation (or confirmation). Such a scenario is not in tune with current trends and needs of increasing velocity in continuous software engineering. In this paper, we propose a tool-supported approach to make security standards more precise and easier to understand for both non-security as well as security experts by applying process models. This approach emerges from a large industrial company and encompasses so far the IEC62443-4-1 standard. We further present a case study with 16 industry practitioners showing how the approach improves communication between development and security compliance practitioners.

==> sections/02_relatedWork.tex <==
\emph{IEC~62443} is a series of standards for IACS security published by the International Electrotechnical Commission (IEC). Part 4-1 describes phases (called practices) for secure product development \cite{IEC41:2018}. We reference this part of the standard as \quotes{4-1} or \quotes{4-1 standard}. 
%\emph{SAFe} is a widely used process framework that scales lean and agile development to large organizations and defines corresponding roles, activities, and artifacts~\cite{Leffingwell:2017}.
Related work discusses using models to derive security activities from regulations, e.g.~\citet{Beckers:2015}. Tthis approach is based on patterns and lacks attention on practical application in industrial environments, e.g. product life cycle~\cite{Cawley:2010}.
% Continuous Software Engineering
%Previous work on \emph{Continuous Software Engineering (CSE)} describes lean and agile principles for continuous \quotes{flow} of activities across business, development, and operations~\cite{Fitzgerald:2017}.

%Authors report compliance and security for continuous development as related but separate concerns~\cite{Fitzgerald:2017,Merkow:2011}. State of the art reports conclude that agile methods are suitable for security-critical environments like IACS but not yet adopted in regulated environments~\citet{Fitzgerald:2013,Cawley:2010}. 
%Practical concerns are adapting the development process to security, eliciting and tracking security requirements in a better way, and incorporating assurance into iterations~\cite{Moyon:2018,Daennart:2019,Villamizar:2018,Baca:2012,Bartsch:2011,Keramati:2008,Beznosov:2004,Siponen:2005}.
% Contribution
For large scale regulated environments, our process models improve comprehension of the top IACS security standard which bridge the gap between software engineering and security compliance~\cite{Jaatun:2017}.
 

\todo{Add references on process models and modelling}
Static Analysis of BPMN-Based Process-Driven Applications \cite{Schneid:2019,Dumas:2010} talk about automatic restructuring, it is not always possible or desirable to have structured models.
